Hierarchical Federated Learning with Privacy

Federated learning (FL), where data remains at the federated clients, and where only gradient updates are shared with a central aggregator, was assumed to be private. Recent work demonstrates that adversaries with gradient-level access can mount successful inference and reconstruction attacks. In such settings, differentially private (DP) learning is known to provide resilience. However, approaches used in the status quo (\ie central and local DP) introduce disparate utility vs. privacy trade-offs. In this work, we take the first step towards mitigating such trade-offs through {\em hierarchical FL (HFL)}. We demonstrate that by the introduction of a new intermediary level where calibrated DP noise can be added, better privacy vs. utility trade-offs can be obtained; we term this {\em hierarchical DP (HDP)}. Our experiments with 3 different datasets (commonly used as benchmarks for FL) suggest that HDP produces models as accurate as those obtained using central DP, where noise is added at a central aggregator. Such an approach also provides comparable benefit against inference adversaries as in the local DP case, where noise is added at the federated clients.

==> macros/defs.tex <==
%%% Some obvious packages to import %%%%
\usepackage{xspace}
\usepackage{xparse}
\usepackage{booktabs}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{scalerel}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\SetMathAlphabet{\mathcal}{bold}{OMS}{cmsy}{b}{n}
\setlength{\topsep}{2pt}

%%% Math mode command / Command to save some space
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{neweqnarrays}}%
\newcommand{\eea}{\end{neweqnarrays}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align*}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align*}}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-1pt}%
\setlength{\belowdisplayskip}{-1pt}%
\setlength{\abovedisplayshortskip}{1pt}%
\setlength{\belowdisplayshortskip}{1pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}


%%% Useful variables and function definitions
\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthat{\: |\:}
\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}
\newcommand{\semi}{\;;\;}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}

\providecommand{\true}{\mathsf{true}}
\providecommand{\false}{\mathsf{false}}
\newcommand{\win}{\mathsf{win}}
\def\negl{\mathsf{negl}}

%% Reference styles
\newcommand{\chapref}[1]{\mbox{Chapter~\ref{#1}}}
\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\apref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\appref}[1]{\apref{#1}}

%\newtheorem{theorem}{Theorem}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\newcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\tabfontsize}{\scriptsize}
\newcommand{\gamesfontsize}{\footnotesize}


%%% Splitting pages for figures and putting border around them
\providecommand{\setstretch}[1]{}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}
\newcommand{\hpagess}[4]{
  \begin{tabular}[t]{c@{\hspace*{.5em}}c}
    \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
    &
      \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
  \end{tabular}
}
\newcommand{\hpagesss}[6]{
  \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
    \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
    &
      \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
    &
      \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
  \end{tabular}
}
\newcommand{\hpagessss}[8]{
  \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
    \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
    &
      \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
    &
      \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
    &
      \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
  \end{tabular}
}

\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
  \begin{tabular}[t]{c@{\hspace*{.3em}}c}
    \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
    &
      \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
  \end{tabular}
}
\newcommand{\hfpagesss}[6]{
  \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
    \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
    &
      \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
    &
      \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
  \end{tabular}
}
\newcommand{\hfpagessss}[8]{
  \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
    \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
    &
      \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
    &
      \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
    &
      \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
  \end{tabular}
}


%%% Other paper specific variables
%% Vectors
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}

\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\bigO}{\mathcal{O}}

\newcommand{\Img}{\textsf{Img}}

\def \Perm {\textsf{Perm}}
\def \mspace {{\mathcal{M}}}
\def \mspacebot {{\mathcal{M}_\bot}}
\def \sspace {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\alphabet}{\Sigma}
\newcommand{\pwchar}{{x}}
\newcommand{\dom}{D}
\newcommand{\domvec}{\vec{D}}
\newcommand{\popdomainsvec}{\vec{D}^*}
\newcommand{\popdomains}{D^*}
\newcommand{\humanornot}{{h}}
\newcommand{\humanornotvec}{\vec{h}}
\newcommand{\ctxtvec}{\vec{C}}


%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {k}
\def \keylen {\kappa}
\def \msg {M}
\def \seed {S}
\def \ctxt {c}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
% \newcommand{\encode}{{\textsf{encode}}}
% \newcommand{\decode}{{\textsf{decode}}}


\newcommand{\DTEuniform}{{\textsf{UNIF}}\xspace}
\newcommand{\encodeuniform}{{\textsf{U-encode}}\xspace}
\newcommand{\decodeuniform}{{\textsf{U-decode}}}

\newcommand{\DTEng}{{\textsf{NG}}\xspace}
\newcommand{\encodeng}{{\textsf{NG-encode}}\xspace}
\newcommand{\decodeng}{{\textsf{NG-decode}}\xspace}

\newcommand{\DTEpcfg}{{\textsf{PCFG}}\xspace}
\newcommand{\encodepcfg}{{\textsf{PCFG-encode}}\xspace}
\newcommand{\decodepcfg}{{\textsf{PCFG-decode}}\xspace}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}

\newcommand{\DTEkamf}{{\small{\sf WEIR-UNIF}}\xspace}
\newcommand{\DTEkamfplus}{{\small{\sf WEIR}}\xspace}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\decodekamfplus}{{\textsf{\KAMFP-decode}}}

% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}

\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}


\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{enc}}}
\def \dec {{\textsf{dec}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\providecommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}


\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {{\mathcal A}}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{G}}} % D
\newcommand{\advDD}{\mathcal{C}}
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\G}{\advG}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

\def\mytablecaption#1{\vspace{2mm}
                      \centerline{Table \arabic{mytable}.~{#1}}
                      \vspace{6mm}
             \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}}


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

\newcommand{\myfigcaption}[1]{
  \vspace{2mm}
  \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
  \vspace{6mm}
  \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%% Formatting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand{\code}{\texttt}
\newcommand{\func}{\textsf}
\newcommand{\variable}{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% New commands:
%
\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
\newtheorem{observation}{Observation}
% \newtheorem{definition}{Definition}
% \newtheorem{claim}{Claim}
% \newtheorem{assumption}{Assumption}
% \newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}

\newcommand{\ts}{t}
\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}

%\newcommand{\note}[2]{\textcolor{red}{Note from #1: #2}}
%\newcommand{\noteari}[1]{\note{Ari}{#1}}

\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}
\newcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
%\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}


\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\thenote: {\sf #1}$\gg$}}}
\newcommand{\mytab}{\hspace*{.4cm}}
\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
% \def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\newcommand{\msglen}{m}
\renewcommand{\SS}{\textsf{SS}\xspace}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Enroll}{\textsf{Enroll}\xspace}
\newcommand{\Entropy}{\textsf{Entropy}\xspace}
\newcommand{\enroll}{\textsf{enroll}\xspace}
\newcommand{\Auth}{\textsf{Authenticate}\xspace}
\newcommand{\auth}{\textsf{authenticate}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}\xspace}
\newcommand{\Ext}{\textsf{Ext}\xspace}
\newcommand{\dis}{\textsf{dis}\xspace}

\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONGUESS}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\newcommand{\return}{\textrm{Return}~}
\def\cs{\ensuremath{t}} % Cache Size
\def\indexj{\ensuremath{\gamma}\xspace}
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\msgspace}{\mathcmd{{\mathcal{M}}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\providecommand{\dist}{\mathcmd{p}}
\newcommand{\pwprob}{\dist}
\newcommand{\w}{{w}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}
\newcommand{\edistname}{{edit distance}\xspace}
\newcommand{\edistcutoff}{\edist}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand{\error}{e}
\newcommand{\tab}[1][1cm]{\hspace*{#1}}
\newcommand{\hatball}{\hat{B}}
\newcommand{\newball}{B^*}
\newcommand{\ballserver}{\tilde{B}}
\newcommand\codewordspace{{\cal C}}
\newcommand\codebook{{C}}


\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\providecommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\w}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
\newcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\newcommand{\typoprob}{\tau}
\def\typodist{\ensuremath{\typoprob_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\PWset}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\providecommand{\supp}{\mbox{supp}}
%\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Exp}{\mathop{\mathbb E}}
%\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
% \providecommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
\newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{\overline{{\footnotesize\textnormal{\textrm{{onguess}}}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onguess}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mkror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{skror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

%\newcommand{\advantage}{\textnormal{\Adv}}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
%\newcommand{\state}{s}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\kk}{k}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{{pk}}
\newcommand{\sk}{{sk}}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textnormal{\textsf{\small Utility}}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\ske}{\mathcal{E}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}
\newcommand{\hlen}{\ell}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
  \setlength{\fboxsep}{-1\fboxrule}
  \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}
}


%% Added for NoCrack
\def\Plus{\texttt{+}}
\def\Minus{\texttt{-}}
\newcommand{\nocrack}{{{N}o{C}rack}\xspace}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\kamf}{Kamouflage\xspace}
\newcommand{\kamfplus}{Kamouflage\Plus\xspace}
\newcommand{\starts}{\texttt{\string^}}
\newcommand{\symend}{\texttt{\$}}
\newcommand{\ngram}{$n$-gram}
\newcommand{\dte}[1]{\texttt{\bf #1}}
\newcommand{\RY}[1]{RY-{#1}}
\newcommand{\pwsalgo}{\textsf{Samp}}


\newcommand{\alphasym}{\texttt{L}}
\newcommand{\digitsym}{\texttt{D}}
\newcommand{\symbolsym}{\texttt{S}}

%% Added for pwtypos
\newcommand{\typocorr}{\text{{T}yp{T}op}\xspace}
%% For name of typos 
\newcommand{\same}{\textsf{same}\xspace}
\newcommand{\swcall}{\textsf{swc-all}\xspace}
\newcommand{\swcfirst}{\textsf{swc-first}\xspace}
\newcommand{\rmlast}{\textsf{rm-last}\xspace}
\newcommand{\rmlastl}{\textsf{rm-lastl}\xspace}
\newcommand{\rmlastd}{\textsf{rm-lastd}\xspace}
\newcommand{\rmlasts}{\textsf{rm-lasts}\xspace}
\newcommand{\rmfirst}{\textsf{rm-first}\xspace}
\newcommand{\dtoslast}{\textsf{n2s-last}\xspace}
\newcommand{\stodlast}{\textsf{s2n-last}\xspace}
% \newcommand{\swslast}{\textsf{sws-last}\xspace}
\newcommand{\keyprox}{\textsf{near-key}\xspace}
\newcommand{\other}{\textsf{other}\xspace}
\newcommand{\upncap}{\textsf{upncap}\xspace}

\newcommand{\typoset}{{\mathcal C}}
\newcommand{\topfive}{{\mathcal C}_{\textrm{top5}}}
\newcommand{\toptwo}{{\mathcal C}_{\textrm{top2}}}
\newcommand{\topthree}{{\mathcal C}_{\textrm{top3}}}
\newcommand{\otherfail}{\textrm{other}}

\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = \tau{op' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = \beta{ottom' strut}}

\def\epwprob{\tilde{\pwprob}}
\def\etypoprob{\tilde{\typoprob}}
\newcommand{\strings}{\calS}
\def\compileskip{1}
\newcommand{\chbudget}{c}
\newcommand{\register}{\textnormal{\textsf{Reg}}\xspace}
\newcommand{\checker}{\textnormal{\textsf{\small Chk}}\xspace}
\newcommand{\checkerall}{\textnormal{\textsf{\small Chk-All}}\xspace}
\newcommand{\checkerbl}{\textnormal{\textsf{\small Chk-wBL}}\xspace}
\newcommand{\checkerapprox}{\textnormal{\textsf{\small Chk-AOp}}\xspace}
\newcommand{\opchecker}{\textnormal{\textsf{\small OpChk}}\xspace}

\newcommand{\exregister}{\textnormal{\textsf{ExReg}}\xspace}
\newcommand{\exchecker}{\textnormal{\textsf{\small ExChk}}\xspace}

\newcommand{\pwlength}{k}
\newcommand{\getpwp}{{\:\leftarrow_{\pwprob}\:}}
\newcommand{\getpw}{{\:\leftarrow_{\pwdist}\:}}
\newcommand{\gettypo}{{\:\leftarrow_{\pw}\:}}
\newcommand{\mut}{f}
\newcommand{\mutset}{F}
\newcommand{\tcf}{g}
\newcommand{\tcfe}{G}
\newcommand{\accept}{{\sf true}}
\newcommand{\reject}{{\sf false}}
\newcommand{\nh}[1]{N(#1)}
\newcommand{\newnh}[1]{N^*_\mutset(#1)}

\newcommand{\ACC}{\textnormal{\textsf{\small ACC}}}
\newcommand{\ATT}{\textnormal{GUESS}}
\newcommand{\CheckOr}{\textnormal{Check}}


%%% Check leaked passwords

\newcommand{\wss}[1]{{\ensuremath{\w_1,\ldots,\w_{#1}}}}
\newcommand{\uwss}[1]{{\ensuremath{(u,\w_1),\ldots,(u,\w_{#1})}}}
\newcommand{\uuwss}[1]{{\ensuremath{(u_1,\w_1),\ldots,(u_{#1},\w_{#1})}}}
\newcommand{\wssin}[2]{{\ensuremath{\w_1,\ldots,\w_{#1}\atop \in #2}}}
\newcommand{\pwold}{\typo}
\newcommand{\negsamplesize}{k\xspace}
\newcommand{\subSampling}{t\xspace}
\newcommand{\mincountvocab}{\ensuremath{v_{\min}}}
\newcommand{\embedding}{E\xspace}
\newcommand{\q}{\ensuremath{q}}
\newcommand{\qbar}{\ensuremath{\bar{q}}}
\newcommand{\param}{\theta}
\newcommand{\grank}{\ensuremath{\beta}}


\def\slack{\mathcmd{m}}
\def\Linf{\mathcmd{W_\infty}}
\def\bucketset{\mathcal{B}}
\newcommand{\buckets}{\ensuremath{{R}}}
\newcommand{\B}{\ensuremath{{\beta}}}
\def\nbuckets{|\bucketset|}

\def\SP{\mathsf{S}}
\def\SPU{\mathsf{\SP_{pu}}}
\def\SPR{\mathsf{\SP_{pr}}}
\def\BC{\B_\mathsf{c}}
\def\PSI{\mathsf{PSI}}
\newcommand{\A}{{\alpha}}
\newcommand{\Abar}{\tilde{\A}^{\vphantom{a}}}
\def\SD{\mathsf{SD}}
\def\bw{\gamma}
\newcommand{\Guessgzero}{\textsf{Guess}}
\newcommand{\AdvGame}[2]{\Adv^{\footnotesize\textnormal{\textrm{#1}}}_{{\footnotesize #2}}}
\newcommand{\Guessgone}{\textsf{BucketGuess}}
\newcommand{\advone}[1]{\AdvGame{\textsf{b-gs}}{#1}}
\newcommand{\advzero}{\AdvGame{\textsf{gs}}{ }}
\newcommand{\zbf}{\ensuremath{\mathbf{z}}}

\newcommand{\allsyms}{\Gamma}
\newcommand{\ijbits}[3]{[#1]_{#2}^{#3}}
\newcommand{\hibp}{\text{HIBP}\xspace}
\newcommand{\goodservice}{\textit{AliceSite.com}\xspace}
\newcommand{\gooduser}{\textit{Bob}\xspace}
\newcommand{\fsbp}{\text{FSB}\xspace}
\newcommand{\ouralgo}{\fsbp}
\newcommand{\google}{\text{GPC}\xspace}
\newcommand{\gpc}{\google}
\newcommand{\idbp}{\text{IDB}\xspace}
\newcommand{\hpbp}{\text{HPB}\xspace}
\newcommand{\hpbpu}{\textsf{$\hpbp_\id$}}
\newcommand{\hpbpw}{\textsf{$\hpbp_\pw$}}
\newcommand{\hpbpuw}{\textsf{$\hpbp_{\id\pw}$}}
\newcommand{\cszero}{\textsf{C3S0}\xspace}
\newcommand{\csone}{\textsf{C3S1}\xspace}
\newcommand{\ccc}{\text{C3}\xspace}
\newcommand{\corrg}{\textsf{Corr-Guess}}
\newcommand{\genguessg}{\textsf{Guess}}
\newcommand{\transform}{\tau}
\newcommand{\bucketg}{\textsf{Bucket-Guess}}

\newcommand{\users}{\mathcal{U}}
\newcommand{\id}{u}
\newcommand{\user}{u}
\newcommand{\usernameT}{\tilde{\user}}
\newcommand{\creds}{\mathcal{S}}
\newcommand{\cred}{s}

\newcommand{\PWleaked}{\tilde{\PW}}
\newcommand{\uleaked}{\tilde{\username}}

\newcommand{\breachDB}{\ensuremath{\tilde{\creds}}}
\newcommand{\breachPW}{\ensuremath{\breachDB_\w}}
\newcommand{\dblen}{N}
\newcommand{\breachU}{\ensuremath{\breachDB_\id}}
\newcommand{\testdata}{\ensuremath{T}}
\newcommand{\sptestdata}{\ensuremath{T_{\text{sp}}}}
\newcommand{\fulldata}{\ensuremath{\calS}}
\newcommand{\guesses}{\ensuremath{L}}

\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\renewcommand{\dist}{\mathcmd{p}}
\newcommand{\distu}{\dist_u}
\newcommand{\distw}{\dist_w}
\newcommand{\dists}{\ensuremath{\distest_s}}
\newcommand{\distn}{\ensuremath{\hat{\dist}_n}}
\newcommand{\dista}{\ensuremath{\distest_a}}
\newcommand{\distest}{\ensuremath{\hat{\mathcmd{p}}}}
\newcommand{\distbreach}{\ensuremath{\hat{\dist}_{h}}}

\def\Bfsb{\B_{\textnormal{\ouralgo}}}
\def\Abarfsb{\Abar_{\ouralgo}}
\def\qdist{\dists(w_{\qbar})}
\newcommand{\prefixlen}{l}
\newcommand{\Ht}[1]{\ensuremath{\H^{(#1)}\xspace}}
\newcommand{\Htl}{\Ht{\prefixlen}}



%%%%%%%%%%%% Add macros relevant for this paper here %%%%%%%%%%%%%%%%%%%%%
\newcommand{\name}{\textsf{OblivTAP}\xspace}
\newcommand{\stap}{\textsf{\name}\xspace}
% \newcommand{\trig}{\mathtt{T}}
% \newcommand{\act}{\mathtt{A}}
\newcommand{\dt}{x}
\newcommand{\payload}{v}
\newcommand{\dtp}{\payload}
\newcommand{\da}{y}
\newcommand{\ei}{e}
\newcommand{\eis}{\ei_s}
\newcommand{\eir}{\ei_r}
\newcommand{\di}{d}
\newcommand{\LT}{X}
\newcommand{\LA}{Y}
\newcommand{\Enc}{\textsf{Enc}\xspace}
\newcommand{\Dec}{\textsf{Dec}\xspace}
\newcommand{\Gb}{\textsf{Gb}}
\newcommand{\Ev}{\textsf{Ev}}
\newcommand{\En}{\textsf{En}}
\newcommand{\De}{\textsf{De}}
\newcommand{\fone}{f_1}
\newcommand{\ftwo}{f_2}
\newcommand{\const}{c}
\newcommand{\cone}{\const_1}
\newcommand{\ctwo}{\const_2}
\newcommand{\Fone}{F_1}
\newcommand{\Ftwo}{F_2}
\newcommand{\TS}{\textsf{TS}\xspace}
\newcommand{\AS}{\textsf{AS}\xspace}
\newcommand{\TAP}{\textsf{TAP}\xspace}
\newcommand{\TC}{\textsf{TC}\xspace}
\newcommand{\PRG}{\textsf{PRG}}
\newcommand{\wlabel}{L}
\newcommand{\encd}{\tilde{d}}

\newcommand{\dfa}{\Gamma}
% \newcommand{\state}{s}
\renewcommand{\trans}{\delta}
\newcommand{\transstring}{{\vec{\delta}}}
\newcommand{\finalstates}{S_F}
\newcommand{\regex}{r}
\newcommand{\nstates}{q}
\newcommand{\Trans}{\Delta}
\newcommand{\Transstring}{{\vec{\Delta}}}
\newcommand{\State}{S}
\newcommand{\state}{s}
\newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\newcommand{\delay}{T}
\newcommand{\sects}{\key_{\scaleto{\TS}{3pt}}}
\newcommand{\secas}{\key_{\scaleto{\AS}{3pt}}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%    END   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> macros/macros.tex <==
% \usepackage{times}  
% \usepackage{hyperref}

% \hypersetup{pdfstartview=FitH,pdfpagelayout=SinglePage}

% \setlength\paperheight {11in}
% \setlength\paperwidth {8.5in}
% \setlength{\textwidth}{7in}
% \setlength{\textheight}{9.25in}
% \setlength{\oddsidemargin}{-.25in}
% \setlength{\evensidemargin}{-.25in}

\usepackage{xspace}
\usepackage{lipsum}% http://ctan.org/pkg/lipsum
\usepackage{graphicx}% http://ctan.org/pkg/graphicx
\usepackage{enumitem}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{color}
\usepackage{tcolorbox}
\usepackage{soul}
\usepackage{float}
\usepackage{mathtools}
\usepackage{subfigure}
\usepackage{amsmath}
\usepackage{cleveref}
\usepackage{authblk}
\pagenumbering{arabic}
\newcommand*{\ie}{{\em i.e.,}\xspace}
\pdfoutput=1

\usepackage{booktabs}
\usepackage{multirow}


%\newcommand*{\ie}{{\em i.e.,}\@\xspace}
\newcommand*{\etal}{{\em et al.}\@\xspace}
\newcommand*{\eg}{{\em e.g.,}\@\xspace}

\newtheorem{claim}{Claim}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}

\newcommand{\varun}[1]{\textcolor{red}{Varun: #1}}
\newcommand{\suman}[1]{\textcolor{green}{Suman: #1}}
\newcommand{\nicolas}[1]{\textcolor{blue}{Nicolas: #1}}

\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
